Perspective of Software Engineering Researchers on Machine Learning Practices Regarding Research, Review, and Education

Context: Machine Learning (ML) significantly impacts Software Engineering (SE), but studies mainly focus on practitioners, neglecting researchers. This overlooks practices and challenges in teaching, researching, or reviewing ML applications in SE. Objective: This study aims to contribute to the knowledge, about the synergy between ML and SE from the perspective of SE researchers, by providing insights into the practices followed when researching, teaching, and reviewing SE studies that apply ML. Method: We analyzed SE researchers familiar with ML or who authored SE articles using ML, along with the articles themselves. We examined practices, SE tasks addressed with ML, challenges faced, and reviewers' and educators' perspectives using grounded theory coding and qualitative analysis. Results: We found diverse practices focusing on data collection, model training, and evaluation. Some recommended practices (e.g., hyperparameter tuning) appeared in less than 20\% of literature. Common challenges involve data handling, model evaluation (incl. non-functional properties), and involving human expertise in evaluation. Hands-on activities are common in education, though traditional methods persist. Conclusion: Despite accepted practices in applying ML to SE, significant gaps remain. By enhancing guidelines, adopting diverse teaching methods, and emphasizing underrepresented practices, the SE community can bridge these gaps and advance the field.

==> 1_preamble.tex <==


\usepackage{acronym}

%---- PACKAGES


\usepackage[inline]{enumitem}
\usepackage{xcolor}
\usepackage{xspace}
\usepackage{booktabs} % For formal tables
\usepackage{soul}
\usepackage[htt]{hyphenat}
\usepackage{tabularx}
\usepackage{tabularray}
\usepackage{natbib}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{url}
\usepackage{placeins}
%----[ Commands ]---
\newcommand{\rev}[1]{\textcolor{blue}{#1}}

%--------Latins
\newcommand{\eg}{\emph{e.g.,}\xspace}
\newcommand{\ie}{\emph{i.e.,}\xspace}
\newcommand{\etal}{\emph{et al.}\xspace}
\newcommand{\aka}{\emph{a.k.a.,}\xspace}
\newcommand{\cf}{\emph{cf.}\xspace}
\newcommand{\mref}{\textcolor{red}{[REF]}\xspace}
\newcommand{\secref}[1]{Section~\ref{#1}\xspace}
\newcommand{\figref}[1]{Fig.~\ref{#1}\xspace}
\newcommand{\tabref}[1]{Table~\ref{#1}\xspace}

% ------------------ Research Questions and challenges
\newcommand{\RQ}[1]{\textbf{RQ$\pmb{_#1}$}}
\newcommand{\RQe}{\emph{RQ}\xspace}
\newcommand{\RQs}{\emph{RQs}\xspace}

\newcommand{\CH}[1]{\textit{CH${_#1}$}}




% ------------------ Variables  
\newcommand{\Var}[1]{\textsf{Var$_#1$}}


% TODO NOTES -------------------------------------------------------------------------------------------------------
\usepackage{lipsum}                     % Dummytext
\usepackage{xargs}                      % Use more than one optional parameter in a new commands
\usepackage[colorinlistoftodos,textsize=small]{todonotes}
\newcommandx{\missing}[2][1=]{\todo[linecolor=red,backgroundcolor=red!25,bordercolor=red,#1]{#2}}
\newcommandx{\change}[2][1=]{\todo[linecolor=blue,backgroundcolor=blue!25,bordercolor=blue,#1]{#2}}
\newcommandx{\info}[2][1=]{\todo[linecolor=OliveGreen,backgroundcolor=OliveGreen!25,bordercolor=OliveGreen,#1]{#2}}
\newcommandx{\improvement}[2][1=]{\todo[linecolor=Plum,backgroundcolor=Plum!25,bordercolor=Plum,#1]{#2}}
\newcommandx{\review}[2][1=]{\todo[linecolor=orange,backgroundcolor=orange!25,bordercolor=orange,#1]{#2}}
\newcommandx{\thiswillnotshow}[2][1=]{\todo[disable,#1]{#2}}


\makeatletter
\if@todonotes@disabled
\newcommand{\hlfix}[2]{#1}
\else
\newcommand{\hlfix}[2]{\texthl{#1}\todo[linecolor=red,backgroundcolor=red!15,bordercolor=red]{#2}}
\fi
\makeatother


%----------------- Commentaries W&M style
\newboolean{showcomments}

% boolean that needs  to be changed for commentaries
\setboolean{showcomments}{true}

\ifthenelse{\boolean{showcomments}}
  {\newcommand{\nb}[2]{
    \fbox{\bfseries\sffamily\scriptsize#1}
    {\sf\small$\blacktriangleright$\textit{#2}$\blacktriangleleft$}
   }
   \newcommand{\cvsversion}{\emph{\scriptsize$-$Id: macro.tex,v 1.9 2005/12/09 22:38:33 giulio Exp $}}
  }
  {\newcommand{\nb}[2]{}
   \newcommand{\cvsversion}{}
  }
\newcommand\DAVID[1]{{\color{blue} \nb{DAVID}{#1}}}
\newcommand\MARIO[1]{{\color{blue} \nb{MARIO}{#1}}}
\newcommand\DENYS[1]{{\color{blue} \nb{DENYS}{#1}}}
\newcommand\TODO[1]{{\color{red} \nb{TODO}{#1}}}




%Inline graphics------------------------------------------------------------------------------------------------------------
\usepackage{graphicx,calc}
\newlength\myheight
\newlength\mydepth
\settototalheight\myheight{Xygp}
\settodepth\mydepth{Xygp}
\setlength\fboxsep{0pt}
\usepackage[]{mdframed}
\usepackage{multirow}
\newcommand*\inlinegraphics[1]{%
	\settototalheight\myheight{Xygp}%
	\settodepth\mydepth{Xygp}%
	\raisebox{-\mydepth}{\includegraphics[height=\myheight]{#1}}%
}

% new commands with inlinegraphics for settings subjects
%\newcommand\SEpapers{\inlinegraphics{case-study2}}
\DeclareRobustCommand{\SEpapers}{\includegraphics[height=2ex]{case-study2}}
\DeclareRobustCommand{\SEcompletepapers}{\includegraphics[height=2ex]{completeSE}}

%\newcommand\SEpapers{\inlinegraphics{case-study}} %light version
%https://www.flaticon.com/free-icon/copy_2874791?term=paper&page=1&position=52&origin=search&related_id=2874791
%\newcommand\SEauthors{\inlinegraphics{pen3}}
\DeclareRobustCommand{\SEauthors}{\includegraphics[height=2ex]{pen3}}
%\newcommand\SEauthors{\inlinegraphics{pen}} %light version
% https://www.flaticon.com/free-icon/paper_2312460?term=paper+and+pen&page=1&position=15&origin=search&related_id=2312460
%\newcommand\SEresearchers{\inlinegraphics{network6}}
\DeclareRobustCommand{\SEresearchers}{\includegraphics[height=2ex]{question}}

%steps labels
\DeclareRobustCommand{\Aone}{\raisebox{-0.2\height}{\includegraphics[height=2.5ex]{A1}}}
\DeclareRobustCommand{\Atwo}{\raisebox{-0.2\height}{\includegraphics[height=2.5ex]{A2}}}
\DeclareRobustCommand{\Athree}{\raisebox{-0.2\height}{\includegraphics[height=2.5ex]{A3}}}
\DeclareRobustCommand{\Afourone}{\raisebox{-0.2\height}{\includegraphics[height=2.5ex]{A41}}}
\DeclareRobustCommand{\Afourtwo}{\raisebox{-0.2\height}{\includegraphics[height=2.5ex]{A42}}}
\DeclareRobustCommand{\Afiveone}{\raisebox{-0.2\height}{\includegraphics[height=2.5ex]{A51}}}
\DeclareRobustCommand{\Afivetwo}{\raisebox{-0.2\height}{\includegraphics[height=2.5ex]{A52}}}

\DeclareRobustCommand{\Bone}{\raisebox{-0.2\height}{\includegraphics[height=2.5ex]{B1}}}
\DeclareRobustCommand{\Btwo}{\raisebox{-0.2\height}{\includegraphics[height=2.5ex]{B2}}}
\DeclareRobustCommand{\Bthree}{\raisebox{-0.2\height}{\includegraphics[height=2.5ex]{B3}}}
\DeclareRobustCommand{\Bfour}{\raisebox{-0.2\height}{\includegraphics[height=2.5ex]{B4}}}
\DeclareRobustCommand{\Bfive}{\raisebox{-0.2\height}{\includegraphics[height=2.5ex]{B5}}}





%\newcommand\SEresearchers{\inlinegraphics{network2}}%light version
%https://www.flaticon.com/free-icon/people_3136102?term=social+network&related_id=3136102
%https://www.flaticon.com/free-icon/contract_598377?term=pen+paper&page=1&position=60&origin=search&related_id=598377

\acrodef{ML}{Machine Learning}
\acrodef{AI}{Artificial Intelligence}
\acrodef{SE}{Software Engineering}
\acrodef{DL}{Deep Learning} 
\acrodef{CsQ+A}[CQ\&A]{Communities of Question and Answers}

\acrodef{ML4SE}[ML4SE]{Machine Learning for Software Engineering} 
%\acrodef{ML4SES}{ML for SE} 
\acrodef{SE4ML}{Software Engineering for Machine Learning}
%\acrodef{ML4SES}{ML for SE} 
\acrodef{SE4AI}{Software Engineering for Artificial Intelligence} 
%\acrodef{SE4MLS}{SE for ML} 
\acrodef{IRR}{inter-rater reliability}

\acrodef{LLM}{Large Language


%----------------  column types with sizes 
\usepackage{array}
\newcommand{\PreserveBackslash}[1]{\let\temp=\\#1\let\\=\temp}
\newcolumntype{C}[1]{>{\PreserveBackslash\centering}p{#1}}
\newcolumntype{R}[1]{>{\PreserveBackslash\raggedleft}p{#1}}
\newcolumntype{L}[1]{>{\PreserveBackslash\raggedright}p{#1}}

%-------- Just to get the width in cm
\usepackage{layouts}
\newcommandx{\qs}[1]{\textit{#1}}
\newcommand{\qstype}[1]{\texttt{#1}}
\newcommand{\qcl}[1]{(\textit{#1})}

%---------------- Commands needed for the appendix

\usepackage{fontawesome}
\usepackage{tasks}
\usepackage{tikz}
\usepackage[usestackEOL]{stackengine}
\usepackage{graphicx}

%Radio buttons
\makeatletter
\newcommand*{\radiobutton}{\@ifstar{\radiobuttonON}{\radiobuttonOFF}}
\makeatother
\def\radiobuttonON{\raisebox{-1.5pt}{\stackinset{c}{}{c}{.35pt}{$\bullet$}{\scalebox{2}{$\circ$}}}}
\def\radiobuttonOFF{\raisebox{-1.5pt}{\scalebox{2}{$\circ$}}}

%Check lists
\newcommand*{\checkboxicon}{$\square$}

% Package for text box 
\usepackage[most]{tcolorbox}
\newtcbox{\inlinebox}[1][]{enhanced,
 box align=base,
 nobeforeafter,
 colback=gray!10,
 colframe=black,
 size=small,
 left=0pt,
 right=0pt,
 boxsep=2pt,
 boxrule=0.5pt,
 #1}

% Text Field  box 
\newcommand{\textfieldtext}{~\inlinebox{\small{\textit{Text\phantom{a}Field}}}~}

% Text Field  numeric  
\newcommand{\textfieldnum}{~\inlinebox{\phantom{T}\#\phantom{T}}~}

% Text Field  others  
\newcommand{\emptyboxOthers}{~\inlinebox{\small{\phantom{This is my}}}~}

